From Orchestration to Choreography through Contract Automata

We study the relations between a contract automata and an interaction model. In the former model, distributed services are abstracted away as automata - oblivious of their partners - that coordinate with each other through an orchestrator. The interaction model relies on channel-based asynchronous communication and choreography to coordinate distributed services. We define a notion of strong agreement on the contract model, exhibit a natural mapping from the contract model to the interaction model, and give conditions to ensure that strong agreement corresponds to well-formed choreography.

==> eptcsdata.tex <==
\providecommand{\firstpage}{67}
\providecommand{\publicationstatus}{I. Lanese, A. Lluch Lafuente, A. Sokolova, H. T. Vieira (Eds.):\\
7th Interaction and Concurrency Experience (ICE 2014)\\
EPTCS 166, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.166.8}{10.4204/EPTCS.166.8}}

